Oscillations of Observables in 1-Dimensional Lattice Systems

Using, and extending, striking inequalities by V.V. Ivanov on the down-crossings of monotone functions and ergodic sums, we give universal bounds on the probability of finding oscillations of observables in 1-dimensional lattice gases in infinite volume. In particular, we study the finite volume average of the occupation number as one runs through an increasing sequence of boxes of size $2n$ centered at the origin. We show that the probability to see $k$ oscillations of this average between two values $\beta $ and $0<\alpha <\beta $ is bounded by $C R^k$, with $R<1$, where the constants $C$ and $R$ do not depend on any detail of the model, nor on the state one observes, but only on the ratio $\alpha/\beta $.

==> fig1.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point 6.2 6.05 {$f(a)$}
\point 8.9 5.8 {$\DD$}
\point 5.65 3.9 {$\CC$}
\point 13.8 7.2 {$f(b)$}
\point 3.05 0.6 {$c$}
\point 6.95 0.6 {$a$}
\point 13.55 0.6 {$b$}
 }}


==> fig2.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point 0.4 -0.4 {$a_j$}
\point 6.1 -0.4 {$b_j$}
\point 3.5 1.2 {\clap{$\Delta_j$}}
\point 6.3 5.2 {$f(b_j)$}
\point 0 3.1 {\llap{$f(a_j)$}}
\point 3.5 2.7 {\clap{$\Delta''_j$}}
\point 6.3 7.5 {$D''_j$}
 }}


==> fig3.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point 0.84 -0.45 {\clap{$a$}}
\point 11.8  -0.45 {\clap{$b$}}
\point  6.25 1.05 {\clap{$\Delta$}}
\point -0.7 3.15 {\llap{$Q(a)$}}
\point 14.8 10.25 {\rlap{$Q(b)$}}
\point 0.5 4.5 {$A$}
\point -1.05 4.35 {\llap{$f(a)$}}
\point 0.5 2.0 {$D$}
\point 11.9 8.1 {$C$}
\point 14.8 8.5 {$f(b)$}
\point 11.9 12.1 {$B$}
\point 2.5 0.4 {$\Delta''$}
\point 3.74 2.0 {$\Delta'$}
\point 13.05 10.25 {\llap{$D''$}}
\point 13.5 10.25 {\rlap{$G(b)$}}
\point 0.5 3.15 {\llap{$G(a)$}}
 }}





